Recent Progress in Conversational AI

Conversational artificial intelligence (AI) is becoming an increasingly popular topic among industry and academia. With the fast development of neural network-based models, a lot of neural-based conversational AI system are developed. We will provide a brief review of the recent progress in the Conversational AI, including the commonly adopted techniques, notable works, famous competitions from academia and industry and widely used datasets.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> hidden.tex <==

\section{Ref from here By Mingda!!!}
1. Ref Blog 
An Annotated Reading List of Conversational AI \cite{Haixun},\\ 
The Stanford Question Answering Dataset\cite{SQuAD}, \\
2. QANet: Combining Local Convolution with Global Self-Attention for Reading Comprehension \cite{qanet},\\
3. Conversational AI chat-bot — Architecture overview\cite{Ravindra}, \\
4. Different Measurements Metrics to Evaluate a Chatbot System\cite{Shawar:2007},\\
5. Deep Reinforcement Learning for Dialogue Generation
\cite{deep-reinforcement-learning-dialogue-generation}, \\
6. Discovering Conversational Dependencies between Messages in Dialogs
\cite{discoverDependencies}, \\

Alexa:
1.UW:  Sounding Board--University of Washington’s Alexa Prize Submission
\cite{fang2017sounding} \\
2.University of Trento:  Roving Mind: a balancing act between open--domain and engaging dialogue systems \cite{alessandra2017roving} \\
3. University of Montreal:

The Octopus Approach to the Alexa Competition: A Deep Ensemble-based Socialbot \cite{octopus}\\
4. University of Edinburgh:

 Edina: Building an Open Domain Socialbot with Self-dialogues \cite{krause2017edina}\\
5. UCSC:

 Slugbot: An Application of a Novel and Scalable Open Domain Socialbot Framework \cite{bowden2018slugbot} \\
6. UCBerkley:

Eigen: A Step Towards Conversational AI \cite{eigen} \\
7.SNU:

 A Chatbot by Combining Finite State Machine, Information Retrieval, and Bot-Initiative Strategy \cite{yichatbot} \\ 
8.RPI:
 A Two-Layer Dialogue Framework For Authoring Social Bots \cite{twoLayer} \\
9. Princeton Pixie: A Social Chatbot  \cite{Pixie} \\
10. HWU Alana: Social Dialogue using an Ensemble Model and a Ranker trained on User Feedback \cite{Alana} \\
11. Emory Emersonbot: Information-Focused Conversational AI Emory University at the Alexa Prize 2017 Challenge \cite{Emersonbot} \\
12. CTU: Alquist: The Alexa Prize Socialbot \cite{Alquist} \\

13. CMU1: \cite{RubyStar} \\
14. CMU2: \cite{CMU} \\
15. Introduction to Alexa Prize: \cite{Intro} \\
General Topics:
1. Conversational AI: The Science Behind the Alexa Prize(2018)
NLP breakthrough:
2017 aaai: SeqGan Combine seq2seq, gan, and reinforcement learning \cite{yu2017seqgan}
2018 aaai: leakGan improve based on seqgan. generator can get more feadback from the discriminator \cite{guo2017long}\\
Work from Facebook AI in 2018
Personalizing dialogue agents: I have a dog, do you have pets too? \cite{zhang2018peron}
In this work, the dialogue agents are grouped into two types: ranking models and generative models


\subsection{Generative Model with Adversarial Training}

Generative adversarial network (GAN) is proposed in~\cite{DBLP:journals/corr/GoodfellowPMXWOCB14}. It achieves excellent performances in fields such as computer vision and graph mining etc. GAN is in the form of generator and discriminator framework. The generator $G$ learns to generate high-quality instances and the discriminator $D$ learns to distinguish whether a generated instance from the generator is real or fake. A number of recent works\cite{yu2017seqgan,guo2017long,DBLP:conf/nips/LinLHSZ17} combine the GAN with the sequence-to-sequence model to build the conversational AI system.

SeqGAN~\cite{yu2017seqgan} applies adversarial training on sequence generation under the reinforcement learning framework. 
SeqGAN models the text generation as a sequential decision-making task. The state is previously generated words, the action is the next word to be generated, and the rewards are the feedback derived from the discriminator. 
More precisely, the generator, constructed by an LSTM model, generates a sequence of words. The generated sequence of words is passed to the discriminator to generate reward signals.
The discriminator is constructed by a binary classifier. The binary classifier takes sentences from real data as positive examples and takes sentences generated by $G$ as negative examples.
The reward is defined by the cross-entropy between the predicted distribution and true distribution.

LeakGAN~\cite{guo2017long} is proposed to address the reward sparsity issue. It further uses features extracted from the discriminator as a step-by-step guide to train the generator. It improves the performance of sequence generation, especially in long text.

RankGAN~\cite{DBLP:conf/nips/LinLHSZ17} claims that the richness inside the sentences constrained by binary prediction is too restrictive and relaxes the training of the discriminator to a learning-to-rank optimization problem.
